FPT Approximation for Constrained Metric $k$-Median/Means

The Metric $k$-median problem over a metric space $(\mathcal{X}, d)$ is defined as follows: given a set $L \subseteq \mathcal{X}$ of facility locations and a set $C \subseteq \mathcal{X}$ of clients, open a set $F \subseteq L$ of $k$ facilities such that the total service cost, defined as $\Phi(F, C) \equiv \sum_{x \in C} \min_{f \in F} d(x, f)$, is minimised. The metric $k$-means problem is defined similarly using squared distances. In many applications there are additional constraints that any solution needs to satisfy. This gives rise to different constrained versions of the problem such as $r$-gather, fault-tolerant, outlier $k$-means/$k$-median problem. Surprisingly, for many of these constrained problems, no constant-approximation algorithm is known. We give FPT algorithms with constant approximation guarantee for a range of constrained $k$-median/means problems. For some of the constrained problems, ours is the first constant factor approximation algorithm whereas for others, we improve or match the approximation guarantee of previous works. We work within the unified framework of Ding and Xu that allows us to simultaneously obtain algorithms for a range of constrained problems. In particular, we obtain a $(3+\varepsilon)$-approximation and $(9+\varepsilon)$-approximation for the constrained versions of the $k$-median and $k$-means problem respectively in FPT time. In many practical settings of the $k$-median/means problem, one is allowed to open a facility at any client location, i.e., $C \subseteq L$. For this special case, our algorithm gives a $(2+\varepsilon)$-approximation and $(4+\varepsilon)$-approximation for the constrained versions of $k$-median and $k$-means problem respectively in FPT time. Since our algorithm is based on simple sampling technique, it can also be converted to a constant-pass log-space streaming algorithm.

==> partition-discussion.tex <==
We would like to make some important observations about the problems mentioned in Table~\ref{table:1}. 
The $r$-gather and $r$-capacity $k$-service problems that we consider in this work is more general than the one considered by Ding and Xu~\cite{Ding_and_Xu_15} in that the  $r_{i}$ values for different clusters may not be the same. 
%It differs from the uniform version of the problem, where every cluster has the same $r_{i}$ value. 
Ding and Xu~\cite{Ding_and_Xu_15} only considered the uniform version of the problem (where all $r_i$'s are the same) and designed a partition algorithm for the same. 
However, their algorithm can easily be generalized for the non-uniform version the we consider.
We describe the algorithm in Section~\ref{section: partition_algm}.
Also note that the last four problems in Table~\ref{table:1}, i.e., fault-tolerant, semi-supervised, uncertain, and outlier $k$-service problems do not satisfy the definition of the constrained $k$-service problem due to which Theorem~\ref{theorem: list_alpha_approx} does not hold for these problems. 
Let us see why.
The fault-tolerant, semi-supervised, and uncertain $k$-service problems have their objective functions different from the one mentioned in Definition~\ref{definition:constrained_k_service}. This distinction is crucial since the list $\mathcal{L}$ only provides a center set, which gives constant approximation with respect to the cost function $\Psi^{*}(\C)$. Therefore, Theorem~\ref{theorem: list_alpha_approx} can not be applied here.
For the outlier $k$-service problem, a feasible clustering is defined over $C \setminus Z$ instead of $C$. Whereas, $\mathcal{L}$ only provide a good center set for the clustering of $C$ and not for $C \setminus Z$. Therefore, Theorem~\ref{theorem: list_alpha_approx} does not work here also.
This problem of misfitting can be evaded by defining these problems differently so that they fit the definition of the constrained $k$-service problem. Let us consider these problems one by one.
\begin{enumerate}
    \item An instance of the fault-tolerant $k$-service problem can be reduced to a special instance of the chromatic $k$-service problem (see section 4.5 of~\cite{Ding_and_Xu_15}). Since we can apply Theorem~\ref{theorem: list_alpha_approx} on the reduced instance, we can also obtain the clustering for the original instance.
    \item For the semi-supervised $k$-service problem, we do not need another equivalent definition. In fact, it can be shown that the list $\mathcal{L}$ provides a good center-set for the objective function $\overline{\Psi}(F,\C) \coloneqq \alpha \cdot \Psi(F,\C) + (1-\alpha) \cdot Dist(\C', \C)$ also (see section 4.4 of~\cite{gjk19}). Therefore, we can apply Theorem~\ref{theorem: list_alpha_approx} on a semi-supervised $k$-service instance.
    \item For the uncertain $k$-service problem, Cormode and McGregor~\cite{2008_cormode} gave an equivalent definition as follows: Given a weighted point set $D \coloneqq \cup_{i = 1}^{n} D_{p}$ such that a point $p_{i} \in D_{p}$  carries a weight of $t_{p}^{i}$, the task is to find a clustering $\mathcal{D} \coloneqq \{D_{1}, D_{2}, \dotsc, D_{k}\}$ of $D$ with minimum $\Psi^{*}(\mathcal{D})$, such that all points in $D_{p}$ are assigned to the same cluster. This definition follows from the linearity of expectation. Moreover, the weighted instance can easily be converted to an unweighted instance by replacing a weighted point with an appropriate number of points of unit weight (see Section 5~\cite{2008_cormode}).
    Now, it fits the definition of the constrained $k$-service problem. Hence, it can be solved using Theorem~\ref{theorem: list_alpha_approx}.
    
    \item At last, we have the outlier $k$-service problem. We do not define the problem differently; instead we construct a new list of center-sets such that it contains a good center-set for any clustering defined over the set $C \setminus Z$ (for any set $Z$ of size $m$).
    However, this new list has a large size, bounded by some function of $k$ and $m$.
    Therefore, the FPT algorithm for the outlier $k$-service problem is parameterized by both $k$ and $m$. On the bright side, we only have $k$ in the exponent term.
    We mention the details of the algorithm in Section~\ref{section:outlier_list_k_service}.
    Since the problem has not been discussed in~\cite{Ding_and_Xu_15}, we mention its partition algorithm in Section~\ref{section: partition_algm}. 
\end{enumerate}
We expect that more problems can fit directly or indirectly in the framework of the constrained $k$-service problem. Since it already encapsulates a wide range of problems, it is important and needful to study this framework properly.
